A Categorical Approach to DIBI Models

The logic of Dependence and Independence Bunched Implications (DIBI) is a logic to reason about conditional independence (CI); for instance, DIBI formulas can characterise CI in probability distributions and relational databases, using the probabilistic and relational DIBI models, respectively. Despite the similarity of the probabilistic and relational models, a uniform, more abstract account remains unsolved. The laborious case-by-case verification of the frame conditions required for constructing new models also calls for such a treatment. In this paper, we develop an abstract framework for systematically constructing DIBI models, using category theory as the unifying mathematical language. In particular, we use string diagrams -- a graphical presentation of monoidal categories -- to give a uniform definition of the parallel composition and subkernel relation in DIBI models. Our approach not only generalises known models, but also yields new models of interest and reduces properties of DIBI models to structures in the underlying categories. Furthermore, our categorical framework enables a logical notion of CI, in terms of the satisfaction of specific DIBI formulas. We compare it with string diagrammatic approaches to CI and show that it is an extension of string diagrammatic CI under reasonable conditions.

==> macros-fossacs.tex <==
% envronment setup
% \AtEndEnvironment{example}{\hfill {\tiny $\blacksquare$}}
\AtEndEnvironment{proof}{\hfill {$\square$}}

\newcommand{\R}[1]{\memSpace{#1}{\val}}
\newcommand{\m}[1]{\mathbf{M}[#1]}
\newcommand{\empmem}{\langle\rangle}

\makeatletter
\newcommand*{\inlineequation}[2][]{%
  \begingroup
    % Put \refstepcounter at the beginning, because
    % package `hyperref' sets the anchor here.
    \refstepcounter{equation}%
    \ifx\\#1\\%
    \else
      \label{#1}%
    \fi
    % prevent line breaks inside equation
    \relpenalty=10000 %
    \binoppenalty=10000 %
    \ensuremath{%
      % \displaystyle % larger fractions, ...
      #2%
    }%
    ~\@eqnnum
  \endgroup
}
\makeatother


\newcommand{\DR}[1]{[#1])}
\newcommand{\PR}[1]{\mathcal{P}(\R{#1})}
\newcommand{\TR}[1]{\funcT(\memSpace{#1}{\val})}
\newcommand{\T}{\mathcal{T}}
\newcommand{\W}[1]{\widehat{f_{#1}}}
\newcommand{\dm}[1]{D_{#1}}
\newcommand{\rg}[1]{R_{#1}}
\newcommand{\dom}{\ensuremath{\mathbf{dom}}}
\newcommand{\range}{\ensuremath{\mathbf{range}}}

\newcommand{\CC}{\mathcal{C}}
\newcommand{\DD}{\mathcal{D}}
\newcommand{\PP}{\mathcal{P}}
\newcommand{\VV}{\mathcal{V}}
\newcommand{\WW}{\mathcal{W}}
\newcommand{\XX}{\mathcal{X}}
\newcommand{\YY}{\mathcal{Y}}
\newcommand{\ZZ}{\mathcal{Z}}

\newcommand{\defeq}{\mathrel{\mathop:}=}
\newcommand{\kl}{\widehat{\odot}}
\newcommand{\pa}{\widehat{\oplus}}
\newcommand{\wh}[1]{\widehat{#1}}
\newcommand{\bomb}{\widehat{!}}
\newcommand{\eeta}{\widehat{\eta}}
% \usepackage{wrapfig}
\def\ci{\perp\!\!\!\perp}
\newcommand{\pearlindep}[3]{\ensuremath{#1 \ci #2 \mid #3}}
    \newcommand{\markovCI}[3]{#1 \!\perp_{\!\mathrm{M}}\! #2 \!\mid\! #3}
    \newcommand{\markovInd}[2]{#1 \!\perp_{\!\mathrm{M}}\! #2}
    \newcommand{\procCI}[3]{#1 \!\perp_{\!\mathrm{S}}\! #2 \!\mid\! #3}
    \newcommand{\procInd}[2]{#1 \!\perp_{\!\mathrm{S}}\! #2}
    \newcommand{\extSupsetCI}[3]{#1 \!\perp_{\!\mathrm{S^+}}\! #2 \!\mid\! #3}
    \newcommand{\probCI}[3]{#1 \!\ci_{\!pr}\! #2 \!\mid\! #3}
    \newcommand{\probInd}[2]{#1 \!\ci_{\!pr}\! #2}
    \newcommand{\dibiCI}[3]{#1 \!\ci_{\!\mathrm{L}}\! #2 \!\mid\! #3}
    \newcommand{\dibiInd}[2]{#1 \!\ci_{\!\mathrm{L}}\! #2}
    \newcommand{\displayCI}[3]{#1 \!\perp\! #2 \!\mid\! #3}
    \newcommand{\displayInd}{\!\perp\!}
\newcommand{\I}[3]{\ensuremath{I(#1, #2, #3)}}

\newcommand{\oran}[1]{\textcolor{orange}{#1}}
\newcommand{\purp}[1]{\textcolor{violet}{#1}}


\newcommand{\jh}[1]{\textcolor{green}{[Justin: {#1}]}}
% \newcommand{\jb}[1]{\ifdraft{\textcolor{brown}{[Jialu: {#1}]}}\fi}
\newcommand{\jb}[1]{\textcolor{brown}{[Jialu: {#1}]}}
\newcommand{\rv}[1]{\textcolor{blue}{[Reviewer: {#1}]}}
\newcommand{\sd}[1]{\ifdraft{\color{red} [Simon: {#1}]}\fi}
\newcommand{\as}[1]{\ifdraft{\color{pink} [A: {#1}]}\fi}
\newcommand{\tao}[1]{\textcolor{purple}{[Tao: {#1}]}}
\newcommand{\fz}[1]{\textcolor{blue} {[Fabio: {#1}]}}
\newcommand{\todo}[1]{\text{\textcolor{red}{TODO: {#1}}}}
\newcommand{\hush}[1]{}
\newcommand{\quieteveryone}{%
	\let\sd\hush%
	\let\jh\hush%
	\let\jb\hush%
	\let\as\hush%
	\let\tao\hush%
	\let\fz\hush%
    \let\todo\hush%
    \let\rv\hush%
}

\newcommand*{\myalign}[2]{\multicolumn{1}{#1}{#2}} %tabular formatting

% \numberwithin{equation}{section}
\usepackage{mathtools}
% do not indent theorems, proofs, definitions, etc.
\makeatletter
\def\@acmplainindent{0pt}
\def\@acmdefinitionindent{0pt}
\def\@proofindent{\noindent}
\makeatother

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% PROGRAMS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \newcommand{\Var}{\ensuremath{\mathsf{Var}}}
\newcommand{\Var}{\setVar}
\newcommand{\Exp}{\ensuremath{\mathsf{Exp}}}
\newcommand{\Com}{\ensuremath{\mathsf{Com}}}
\newcommand{\expWithContext}[2]{{#2}.{#1}}
%\newcommand{\comWithContext}[3]{{\left(#2, #3\right)}.{#1}}
\newcommand{\comWithContext}[3]{#1}

\newcommand{\Val}{\ensuremath{\mathbf{Val}}}

\newcommand{\denot}[1]{\ensuremath{\llbracket #1 \rrbracket}}
    \newcommand{\denotExp}[1]{\llbracket #1 \rrbracket}
\newcommand{\Bool}{\{ 0, 1 \}}
\newcommand{\dbind}{\bind}
\newcommand{\dunit}{\monadUnit{\funcT}{}}
\newcommand{\dcond}[2]{\ensuremath{{#1} \mid {#2}}}
\newcommand{\dconv}[3]{\ensuremath{{#2} \mathbin{\oplus_{#1}} {#3}}}
\newcommand{\kconv}[3]{\ensuremath{{#2} \mathbin{\overline{\oplus}_{#1}} {#3}}}

\newcommand{\ktt}{\ensuremath{\mathit{tt}}}
\newcommand{\kff}{\ensuremath{\mathit{ff}}}
\newcommand{\FV}{\ensuremath{\text{FV}}}
\newcommand{\RV}{\ensuremath{\text{RV}}}
\newcommand{\WV}{\ensuremath{\text{WV}}}
\newcommand{\MV}{\ensuremath{\text{MV}}}
\newcommand{\FFV}{\ensuremath{\text{FV}_{\text{D}}}}
\newcommand{\SFV}{\ensuremath{\text{FV}_{\text{R}}}}

\newcommand{\Skip}{\mathbf{skip}}
\newcommand{\Seq}[2]{{#1} \mathrel{;} {#2}}
\newcommand{\Assn}[2]{\ensuremath{{#1} \leftarrow {#2}}}
\newcommand{\Rand}[2]{{#1} \stackrel{\raisebox{-.25ex}[.25ex]%
{\tiny $\mathdollar$}}{\raisebox{-.2ex}[.2ex]{$\leftarrow$}} {#2}}
\newcommand{\DCond}[3]{\mathbf{if}_D\ #1\ \mathbf{then}\ #2\ \mathbf{else}\ #3}
\newcommand{\DCondt}[2]{\mathbf{if}_D\ #1\ \mathbf{then}\ #2}
\newcommand{\DFor}[4]{\mathbf{for}\ #1 = #2, \dots, #3\ \mathbf{do}\ #4}
\newcommand{\DWhile}[2]{\mathbf{while}\ #1\ \mathbf{do}\ #2}
\newcommand{\RCond}[3]{\mathbf{if}_R\ #1\ \mathbf{then}\ #2\ \mathbf{else}\ #3}
\newcommand{\RCondt}[2]{\mathbf{if}_R\ #1\ \mathbf{then}\ #2}
\newcommand{\Cond}[3]{\mathbf{if}\ #1\ \mathbf{then}\ #2\ \mathbf{else}\ #3}
\newcommand{\Condt}[2]{\mathbf{if}\ #1\ \mathbf{then}\ #2}
% \newcommand{\RWhile}[2]{\mathbf{while}_R\ #1\ \mathbf{do}\ #2}

\newcommand{\MonadExpr}[1]{\ulcorner #1 \urcorner}
\newcommand{\CondChoice}[3]{#2 +_{#1} #3}

\newcommand\Field{\textsf{Field}}
\newcommand\Researcher{\textsf{Researcher}}
\newcommand\Conference{\textsf{Conference}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% SEP LOGIC %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\LOGIC}{DIBI\xspace}
\newcommand{\RLOGIC}{R\LOGIC}
\newcommand{\SYSTEM}{MCSL\xspace}
\newcommand{\ExONE}{\textsc{CommonCause}\xspace}
\newcommand{\ExTWO}{\textsc{CondSamples}\xspace}
\newcommand\sepid{\ensuremath{I}}

% \usepackage{bbding}%\EightAsterisk \SixFlowerPetalDotted
\newcommand\sepand{\mathrel{\ast}}
\newcommand\sepimp{\mathrel{-\mkern-6mu*}}
\newcommand{\bigsep}{\mathop{\Huge \mathlarger{\mathlarger{*}}}}

\newcommand\depid{\ensuremath{J}}



\newcommand\depand{\fatsemi}%\mathrel{;}}
\newcommand\depimpr{\mathrel{\multimap}}
\newcommand\depimpl{\mathrel{\multimapinv}}

\newcommand{\MD}{\ensuremath{M^{D}}}
\newcommand{\MP}{\ensuremath{M^{P}}}
\newcommand{\MS}{\ensuremath{M^{S}}}
\newcommand{\M}{M}

\newcommand{\rseq}{\mathbin{-\mkern-2mu\triangleright}} %right implication for sequential composition
\newcommand{\lseq}{\mathbin{\triangleright\mkern-2mu-}}
\newcommand{\PrimePredicate}[2]{P(#1) = \begin{cases} 1 & \text{if } #2 \\ %Prime Predicate
				0 & \text{otherwise} \end{cases}}

\newcommand{\Bern}{\ensuremath{\mathbf{B}}}
\newcommand{\Dist}{\ensuremath{}}
\newcommand{\distA}{\mu}
\newcommand{\Exact}[1]{#1}
\newcommand{\kp}[2]{\ensuremath{{#1} \mathrel{\triangleright} [{#2}]}}
\newcommand{\pair}[2]{\kp{\Exact{#1}}{\Dist{[#2]}}}
\newcommand{\empdom}[1]{\kp{\Exact{\emptyset}}{#1}}
\newcommand{\indep}[3]{ [#1] \depand ([#2] \sepand [#3])}

\newcommand{\psl}[3]{\{ #1 \}\ #2\ \{ #3 \}}
\newcommand{\bind}{\textsf{bind}}
\newcommand{\unit}{\textsf{unit}}
\newcommand{\Kl}{\mathcal{K}\mkern-2mu\ell}
\newcommand{\Frestrict}{\mathrm{Form_{\RLOGIC}}}
\newcommand{\kernelWithType}[3]{(#2, #3).{#1}}

%%%%%%%%%%%%%%%
%Below is some macros defined by Tao for temporary usage. To be cleaned up later.
\newcommand{\stPlus}{\oplus}
\newcommand{\stThen}{\mathbin{\odot}}
\newcommand{\stUnit}[1]{\mathsf{Unit}_{#1}}
\newcommand{\stLarger}{\sqsupseteq}
\newcommand{\stSmaller}{\sqsubseteq}
    \newcommand{\stLeq}{\sqsubseteq}
    \newcommand{\stGeq}{\sqsupseteq}
\newcommand{\frameX}
{\mathcal{X}}
\newcommand{\frameA}{\mathcal{A}}
\newcommand{\unitSet}{E}
\newcommand{\powset}{\mathcal{P}}
\newcommand{\fpowset}{\mathcal{P}_{\!\!f}}
\newcommand{\ipowset}{\powset_{\!i}}
    \newcommand{\fipowset}{\powset_{\!fi}}
\newcommand{\onlyif}{\Longrightarrow}
\newcommand{\catC}{\mathbb{C}}
\newcommand{\catD}{\mathbb{D}}
\newcommand{\catX}{\mathbb{X}}
\newcommand{\funcF}{\mathcal{F}}
\newcommand{\funcG}{\mathcal{G}}
\newcommand{\funcH}{\mathcal{H}}

\newcommand{\obX}{\mathsf{X}}
    \newcommand{\obY}{\mathsf{Y}}
    \newcommand{\obZ}{\mathsf{Z}}
    \newcommand{\obU}{\mathsf{U}}
    \newcommand{\obV}{\mathsf{V}}
    \newcommand{\obW}{\mathsf{W}}
    \newcommand{\obC}{\mathsf{C}}
    \newcommand{\obD}{\mathsf{D}}
    \newcommand{\obA}{\mathsf{A}}
    \newcommand{\obB}{\mathsf{B}}
    \newcommand{\obE}{\mathsf{E}}

\newcommand{\catSyn}{\mathsf{Syn}}
    \newcommand{\catSynCD}{\catSyn^{CD}}
    \newcommand{\catSynMarkov}{\catSyn^{\mathit{Mkv}}}
    \newcommand{\catSynKernelMarkov}{\mathsf{SynKer}^{\mathit{Mkv}}}
    \newcommand{\catSynKernelCD}{\mathsf{SynKer}^{\mathit{CD}}}
    \newcommand{\catSemKernel}[1]{\mathsf{Ker}(#1)}
\newcommand{\tensor}{\otimes}
\newcommand{\tenUnit}{\mathsf{I}}
\newcommand{\lr}[1]{\langle #1 \rangle}
\newcommand{\lrangle}[1]{\langle #1 \rangle}
\newcommand{\copyMor}{\mathsf{copy}}
% \newcommand{\copier}[1][]{\copyMor_{#1}}
\newcommand{\copier}{\tikzfig{copier}}
\newcommand{\discardMor}{\mathsf{del}}
% \newcommand{\discarder}[1][]{\discardMor_{#1}}
\newcommand{\discarder}{\tikzfig{discarder}}
\newcommand{\unitMor}{
\begin{tikzpicture}[scale = 1, baseline = 1pt]
	\coordinate (1) at (0pt, 4pt);
	\coordinate (2) at (7pt, 4pt);
	%\coordinate (5) at (0pt, 8pt);
	%\coordinate (6) at (8pt, 8pt);
	\draw (1) to (2);
	%\draw[white] (5) to (6);
	\filldraw[fill=black] (1) circle[radius = 1.5pt];
\end{tikzpicture}
}
\newcommand{\codiscarder}[1][]{\unitMor_{#1}}
\newcommand{\symMor}{\sigma}
\newcommand{\swap}{\tikzfig{swap}}
\newcommand{\catFrame}[1]{\frameX_{#1}}
    \newcommand{\catState}[1]{X_{#1}}
\newcommand{\ob}[1]{\mathbf{ob}(#1)}
    \newcommand{\mor}[1]{\mathbf{mor}(#1)}
\newcommand{\id}{\mathit{id}}
    \newcommand{\idMor}{\mathit{id}}
\newcommand{\after}{\circ}
\newcommand{\setVar}{\mathrm{Var}}
\newcommand{\frameSD}{\mathcal{M}}
    \newcommand{\stateSD}{M}
    \newcommand{\unitSD}{M} %the set of unites for \frameSD
\newcommand{\strd}[1]{\scalebox{0.6}{\tikzfig{#1}}} %insert tikzfig inline
\newcommand{\freeCD}[2]{\mathsf{freeCD}(#1, #2)}
\newcommand{\genOb}[1][]{X_{#1}}
\newcommand{\genMor}[1][]{\Sigma_{#1}}
\newcommand{\genBox}[2]{d^{#1}_{#2}}
\newcommand{\varLeq}{\preceq}
    \newcommand{\varLessThan}{\prec}
\newcommand{\funcT}{\mathcal{T}}
\newcommand{\stren}{\mathsf{st}}
    \newcommand{\doublest}{\mathsf{dst}}
\newcommand{\catSet}{\mathsf{Set}}
    \newcommand{\catRel}{\mathsf{Rel}}
    \newcommand{\catPartOrder}{\mathsf{Poset}}
\newcommand{\nomSet}{\mathbf{Nom}}
\newcommand{\setOne}{\mathbf{1}}
\newcommand{\frameM}[1][]{\mathsf{Ker}(#1)}
    \newcommand{\frameMVar}[1][]{\mathsf{Ker}_{\vLeq}(#1)}
\newcommand{\frameMulset}[1]{M^{#1}_{\setVar}}
\newcommand{\setVal}{\mathrm{Val}}
\newcommand{\decomp}[1]{\lr{#1}}
% \newcommand{\then}{\mathrel{;}}
% \newcommand{\then}{;\mkern-2mu}
\newcommand{\then}{\boldsymbol{;}}
\newcommand{\domain}[1]{\mathit{dom}(#1)}
\newcommand{\codom}[1]{\mathit{cod}(#1)}
\newcommand{\disjoint}{\not\cap}
\newcommand{\eql}[1]{\stackrel{\mathclap{\mbox{$\scriptstyle #1$}}}{=}}
\newcommand{\emptyList}{[~]}
\newcommand{\stEq}{\approx}
\newcommand{\eqCl}[2]{[#1]_{#2}}
\newcommand{\eCl}[1]{\left[#1\right]}
\newcommand{\dst}{\text{dst}}
\newcommand{\indstr}{\mathcal{I}}
\newcommand{\iso}{\cong}
\newcommand{\ket}[1]{|#1\rangle}
\newcommand{\inv}[1]{\overleftarrow{#1}}
\newcommand{\dist}{\mathcal{D}}
    \newcommand{\subdist}{\dist_{\leq}}
\newcommand{\supp}{\mathit{supp}}
\newcommand{\empset}{\varnothing}
\newcommand{\FinProb}{\mathbf{FinProb}}
\newcommand{\FinSur}{\mathbf{FinSur}}
\newcommand{\HeapV}{\mathbf{Heap(V)}}
	\newcommand{\HeapVNew}{\mathbf{Heap(V)'}} % not a good notation; needs to change
\newcommand{\Loc}{\mathrm{Loc}}
\newcommand{\val}{\mathrm{val}}
\newcommand{\bool}{\mathrm{bool}}
\newcommand{\wit}{\iota}
\newcommand{\partinj}{\rightharpoonup} % not the exact notation; needs to change
%\newcommand{\partinj}{\hookrightarrow}
\newcommand{\upright}{\upharpoonright}
\newcommand{\binv}[2]{(#1)^{\dagger}_{#2}}
    \newcommand{\bayinv}[1]{{#1}^\dagger}
\newcommand{\catE}{\mathbf{E}}
\newcommand{\coslice}[2]{{#1} / {#2}}
    \newcommand{\slice}[2]{{#1} \backslash {#2}}
\newcommand{\indset}[1]{\mathbf{#1}}
\newcommand{\pState}[1]{\omega_{#1}}
\newcommand{\indepSetI}{\mathcal{I}}
    \newcommand{\condindepSetI}[1]{\mathcal{I}_{#1}}
\newcommand{\bigtensor}{\bigotimes}
% \newcommand{\memproj}[2]{{#1} \!\upharpoonright\! {#2}}
\newcommand{\newtensor}{\boxplus}
    \newcommand{\newtensorunit}{    J}
\newcommand{\copytensor}{\triangle}
\newcommand{\set}[1]{\mathcal{#1}}
\newcommand{\catFullKlP}{\mathbf{A}}
%\newcommand{\supp}{\mathit{supp}}
\newcommand{\catA}{\mathbf{A}}
\newcommand{\natJoin}{\bowtie}
\newcommand{\joinDep}{\bowtie}
\newcommand{\setAttr}{\mathrm{Attr}}
\newcommand{\relProj}[2]{{#1}^{#2}}
    \newcommand{\tupProj}[2]{{#1}^{#2}}
    \newcommand{\tupJoin}{\bullet}
\newcommand{\proj}{\pi}
\newcommand{\distProj}[2]{{#1}^{#2}}
\newcommand{\memProj}[2]{{#1}^{#2}}
\newcommand{\srM}{\mathcal{M}}
    \newcommand{\srPlus}{+}
    \newcommand{\srZero}{0}
    \newcommand{\srTimes}{\times}
    \newcommand{\srOne}{1}
\newcommand{\srTwo}{\mathbf{2}}
    \newcommand{\setTwo}{\mathbf{2}}
\newcommand{\monoidM}{\mathcal{M}}
    \newcommand{\monPlus}{+}
    \newcommand{\monZero}{0}
\newcommand{\natN}{\mathbb{N}}
\newcommand{\funcMSet}[1]{\mathcal{T}_{#1}}
\newcommand{\mand}{*}
\newcommand{\mimp}{\mathrel{-\mkern-6mu*}}
\newcommand{\biThen}{\mathbin{\fatsemi}}
\newcommand{\biTo}{\multimap}
    % \newcommand{\biOt}{\multimapinv}
    \newcommand{\biOt}{\mathrel{\reflectbox{$\multimap$}}}
\newcommand{\selectOb}{\phi}
\newcommand{\vLeq}{\preceq}
\newcommand{\tensorMinus}{-}
\newcommand{\klto}{\rightarrowtriangle}
\newcommand{\emptydist}{\varnothing}
\newcommand{\memoryL}{\bm{\ell}}
\newcommand{\memoryM}{\mathbf{m}}
\newcommand{\memoryN}{\mathbf{n}}
\newcommand{\fsubseteq}{\subseteq_{\!f}\!}
\newcommand{\monadUnit}[2]{\eta^{#1}_{#2}}
    \newcommand{\monadMult}[2]{\mu^{#1}_{#2}}
\newcommand{\attr}[1]{\mathbf{#1}}
\newcommand{\tupSet}[1]{\mathbf{Tup}[#1]}
\newcommand{\setAtomProp}{\mathcal{AP}}
\newcommand{\smallDIBI}{\ensuremath{\text{DIBI}_{\{\land, \mand, \biThen\}}}}
\newcommand{\valV}{\mathcal{V}}
    \newcommand{\natVal}{\mathcal{V}_{\mathrm{nat}}} % i found it more intuitive to use V for valuations
\newcommand{\satisfy}[1]{\vDash_{#1}}
\newcommand{\sampleCoin}{\Omega_{coin}}
\newcommand{\mulspanCol}[1]{\mathcal{#1}}
\newcommand{\indProd}{\bigoplus}
\newcommand{\asind}[1]{\ci_{AS} {#1}}
\newcommand{\indProj}{\pi}
\newcommand{\setGift}{\mathsf{Gift}}
    \newcommand{\candy}{\mathsf{candy}}
    \newcommand{\choco}{\mathsf{choco}}
    \newcommand{\cookie}{\mathsf{cookie}}
\newcommand{\setBox}{\mathsf{Color}}
    \newcommand{\boxR}{\mathsf{red}}
    \newcommand{\boxB}{\mathsf{blue}}
    \newcommand{\boxG}{\mathsf{green}}
    \newcommand{\boxY}{\mathsf{yellow}}
\newcommand{\catRV}[1]{\mathsf{RV}(#1)}
    \newcommand{\catRVDist}{\mathbf{D}}
\newcommand{\valTo}{\Rightarrow}
\newcommand{\valSpace}[1]{\mathbf{Val}(#1)}
\newcommand{\memSpace}[2]{\mathbf{M}[#1; #2]}
    \newcommand{\memSpaceS}[1]{\mathbf{M}[#1]}
    \newcommand{\memSpaceCont}[1]{\mathsf{M}^{\monadGiry}(#1)}
\newcommand{\valA}{\mathit{s}}
\newcommand{\valB}{\mathit{t}}
% \newcommand{\Values}[1]{\mathit{Val}_{#1}}
\newcommand{\Values}{\mathrm{Val}}
\newcommand{\varList}[1]{\llparenthesis #1 \rrparenthesis}
    \newcommand{\setToList}[1]{\llbracket #1 \rrbracket}
\newcommand{\varListMinus}{-}
\newcommand{\xeq}[1]{\stackrel{#1}{=}}
\newcommand{\xleq}[1]{}
\newcommand{\eqWhenDefined}{\doteq}

\newcommand{\catVarWithVal}[3]{#1(#2, #3)}
\newcommand{\catWithVarName}[2]{#1[#2]}
\newcommand{\obChoice}{\theta}
\newcommand{\catSynVar}{\mathbb{SynVar}}
\newcommand{\catKernel}[1]{\mathbb{Ker}(#1)}
\newcommand{\catMemProb}{\mathbb{MemPr}}

% macros for relational lifting of categories;
\newcommand{\relLiftCat}{Rel}
\newcommand{\tensorAnother}{\hat{\otimes}}
    \newcommand{\tenUnitAnother}{\hat{I}}
\newcommand{\tenAss}{\alpha}
    \newcommand{\tenAssAnother}{\hat{\alpha}}
\newcommand{\tenUnitLeft}{\lambda}
    \newcommand{\tenUnitLeftAnother}{\hat{\lambda}}
\newcommand{\tenUnitRight}{\rho}
    \newcommand{\tenUnitRightAnother}{\hat{\rho}}
\newcommand{\tenSwap}{\sigma}
    \newcommand{\tenSwapAnother}{\hat{\sigma}}
\newcommand{\idMorAnother}{\hat{\idMor}}
\newcommand{\afterAnother}{\hat{\after}}
\newcommand{\funcComb}{\mathsf{Comb}}
\newcommand{\funcFreeSetOfFunc}{\mathsf{Free}}
\newcommand{\kernelInduce}[2]{{#1}_{#2}}
% \newcommand{\setProbKern}[2]{\mathbf{Ker}({#1}, {#2})}

% probkernels
\newcommand{\setProbKern}[1]{\mathit{ProbKer}({#1})}
% \newcommand{\conProbKern}{\mathit{ConProbKer}}
\newcommand{\conProbKern}{\mathrm{ProbKer}}
\newcommand{\conTKern}{\mathit{ConTKer}}
\newcommand{\partialTo}{\rightharpoonup}
\newcommand{\obVal}[1]{\mathsf{Val}_{#1}}
% \newcommand{\operateVar}{\mathbin{\spadesuit}}
\newcommand{\operateVar}{\star}
\newcommand{\listL}{L}
\newcommand{\listK}{K}
\newcommand{\setSynKernel}{\mathit{SynKer}}
    \newcommand{\frameSynKernel}{\mathbf{SynFr}}
    \newcommand{\setSemKernel}[1]{\mathrm{Ker}(#1)}
    % \newcommand{\frameSemKernel}[1]{\mathcal{K}\!\mathit{er}(#1)}
    % \newcommand{\frameSemKernel}[1]{\mathcal{K}\mkern-2mu\mathit{er}(#1)}
    \newcommand{\frameSemKernel}[1]{\mathbf{Fr}(#1)}
    \newcommand{\setSynKernelCD}{\mathrm{SynKer^{CD}}}
    \newcommand{\probFrame}{\mathbf{PrFr}}
    \newcommand{\probFrameBasedOn}[1]{\mathbf{PrFr}[#1]}
\newcommand{\listx}{\bar{x}}
\newcommand{\listy}{\bar{y}}
\newcommand{\listu}{\bar{u}}
\newcommand{\listv}{\bar{v}}
\newcommand{\listw}{\bar{w}}
\newcommand{\lists}{\bar{s}}
\newcommand{\listt}{\bar{t}}
\newcommand{\listz}{\bar{z}}
\newcommand{\listCup}{\sqcup}
\newcommand{\listCap}{\sqcap}
\newcommand{\sublist}{\subset}
\newcommand{\sublisteq}{\subseteq}
\newcommand{\sublisteqi}{\subseteq_{i}}
\newcommand{\probKernToDKern}{\alpha}
\newcommand{\DKernToProbKern}{\beta}
\newcommand{\valSpaceToProd}{\iota}
\newcommand{\prodToValSpace}{\iota^{-1}}
\newcommand{\catProbKern}{\mathbb{PrKern}}
\newcommand{\tupleMem}[1]{\overrightarrow{#1}}

% multiset kernel
\newcommand{\funcBag}{\mathcal{B}}
% \newcommand{\conMultKern}{\mathit{ConMultKer}}
\newcommand{\conMultKern}{\mathrm{MultKer}}

% Commands added for CPSL
\newcommand{\monadVal}{M}

% Example of multirelation
\newcommand{\varCustomer}{\mathtt{customer}}
\newcommand{\varProduct}{\mathtt{product}}
\newcommand{\varPrice}{\mathtt{price}}
\newcommand{\valCustomer}{\mathtt{Customer}}
\newcommand{\valProduct}{\mathtt{Product}}
\newcommand{\valPrice}{\mathtt{Price}}
\newcommand{\Alice}{\mathtt{Alice}}
\newcommand{\Bob}{\mathtt{Bob}}
\newcommand{\Tissue}{\mathtt{Tissue}}
\newcommand{\Soap}{\mathtt{Soap}}
\newcommand{\Towel}{\mathtt{Towel}}

% category of dibi frames
% \newcommand{\catDibiFrame}{\mathsf{FrameDIBI}}
\newcommand{\catDibiFrame}{\mathbb{DibiFr}}
\newcommand{\catProbFrame}{\mathbb{PrFr}}
\newcommand{\catTFrame}{\mathbb{TFrame}}
\newcommand{\catKlDFrame}{\Kl(\dist)\mathsf{Frame}}
\newcommand{\catKlTFrame}{\Kl(\funcT)\mathsf{Frame}}
\newcommand{\probframe}{\mathcal{X}_{\mathsf{Prob}}}
\newcommand{\concreteTframe}{\mathcal{X}_{\mathsf{concrete}}}
\newcommand{\KLDframe}{\mathcal{X}_{\dist}}
\newcommand{\KLTframe}{\mathcal{X}_{\funcT}}
\newcommand{\KlDframe}{\KLDframe}
\newcommand{\funcKlDtoProbFrame}{I}
\newcommand{\funcProbtoKlDFrame}{J}

% sets 
\newcommand{\setX}{X}
\newcommand{\setY}{Y}

% continuous model 
\newcommand{\borel}{\mathcal{B}}
\newcommand{\real}{\mathbb{R}}
\newcommand{\catMeas}{\mathbb{Meas}}
\newcommand{\spaceX}{\mathscr{X}}
    \newcommand{\spaceY}{\mathscr{Y}}
    \newcommand{\spaceZ}{\mathscr{Z}}
\newcommand{\sigalg}[1]{\Sigma_{\!{#1}}}
\newcommand{\monadGiry}{\mathcal{G}}
\newcommand{\monadRadon}{\mathcal{R}}
\newcommand{\ev}{\text{ev}}
\newcommand{\dirac}[1]{\delta_{#1}}
\newcommand{\catStoch}{\mathbb{Stoch}}
\newcommand{\catHaus}{\mathbb{CHaus}}
\newcommand{\catGauss}{\mathbb{Gauss}}
\newcommand{\catBorelStoch}{\mathbb{BorelStoch}}
\newcommand{\catRadon}{\mathbb{Radon}}
\newcommand{\emptyele}{\lrangle{}}
\newcommand{\uniform}{\textsc{Unif}}

\newcommand{\trivList}{\langle \rangle}
\newcommand{\normal}{\mathcal{N}}
\newcommand{\cov}{\sigma^2}
\newcommand{\EE}{\mathbb{E}}
% \newcommand{\Var}{\mathbb{Var}} % for covariance
\newcommand{\initialMap}{!}

\newcommand{\isDefined}{\!\Downarrow\!}
\newcommand{\eqIfDefined}{\doteq}
\newcommand{\support}[1]{\mathrm{supp}(#1)}
\newcommand{\memComb}{\uplus}




==> packages-fossacs.tex <==
\usepackage{color, colortbl}
\usepackage{stmaryrd}
\usepackage{amsmath,amssymb}
\usepackage{bm}
\usepackage[all]{xy} %draw commutative diagram
\usepackage{xfrac}
\usepackage{tikz,tikzit}
    \input{local.tikzstyles}
% \usepackage{txfonts}
\usepackage{algpseudocode}
\usepackage{mathpartir}
\usepackage{xspace}
\usepackage{hyperref}
\usepackage{multicol}
\usetikzlibrary{patterns}
\usepackage{wrapfig}
\usepackage{graphicx}
\usepackage{cleveref}
% \usepackage{subfigure}
\usepackage{subcaption}
\usepackage[inline]{enumitem}
\usepackage{mathrsfs}
\usepackage{mathbbol}
% line numbers
\usepackage{lineno}
\usepackage{thm-restate}
\usepackage{mathdots}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{cutwin}

